DotHash: Estimating Set Similarity Metrics for Link Prediction and Document Deduplication

Metrics for set similarity are a core aspect of several data mining tasks. To remove duplicate results in a Web search, for example, a common approach looks at the Jaccard index between all pairs of pages. In social network analysis, a much-celebrated metric is the Adamic-Adar index, widely used to compare node neighborhood sets in the important problem of predicting links. However, with the increasing amount of data to be processed, calculating the exact similarity between all pairs can be intractable. The challenge of working at this scale has motivated research into efficient estimators for set similarity metrics. The two most popular estimators, MinHash and SimHash, are indeed used in applications such as document deduplication and recommender systems where large volumes of data need to be processed. Given the importance of these tasks, the demand for advancing estimators is evident. We propose DotHash, an unbiased estimator for the intersection size of two sets. DotHash can be used to estimate the Jaccard index and, to the best of our knowledge, is the first method that can also estimate the Adamic-Adar index and a family of related metrics. We formally define this family of metrics, provide theoretical bounds on the probability of estimate errors, and analyze its empirical performance. Our experimental results indicate that DotHash is more accurate than the other estimators in link prediction and detecting duplicate documents with the same complexity and similar comparison time.

==> content/results.tex <==
\section{Results}
\label{sec:results}

In this section we show the results of the link prediction experiment. The accuracy results are shown in Figure~\ref{fig:link-pred-hits}, where we can depict three charts showing the Hits@K for each dataset as the dimensions, used for estimating the link prediction task, increase. For every dataset we have the Hits@K, of the precise Adamic-Adar prediction. For both the Drugs (ogbl-ddi) and Proteins (ogbl-ppa) dataset, we have that the estimation of Adamic-Adar gives the best result and reaches the same accuracy as the precise Adamic-Adar computation, which can only be achieved by \ourhash{}. For the Jaccard estimation we see that \ourhash{} and MinHash end up having the same accuracy when the number of dimensions is high enough, however MinHash tends to reach the best accuracy with a lower number bear in mind that for MinHash, dimensions mean the number of hashing functions used and for \ourhash{} it refers to the size of the tensors used. Lastly we have the Collab (ogbl-collab) dataset, that the estimation using MinHash reaches the highest point with fewer dimensions compared to \ourhash{} for both Jaccard and Adamic-Adar. For every dataset SimHash performed the worst. Overall we can observe that the dataset with a bigger median degree proved to perform better for the estimation of Adamic-Adar and reach the best Accuracy for Jaccard with fewer dimensions. 

\subsection{Jaccard estimation}
The results of this experiment can be depicted in \pere{Figure x} in \pere{Appendinx}. This results are important and meaningful, however for the scope of this paper we have decided to put them in the Annex. The results show that MinHash, has always the minimum error for all the datests with the minimum number of dimensions, however as mentioned previously the dimensions for \ourhash{} and MinHash do not represent the same, and this provokes that MinHash take more time at estimating the Jaccard index for the same number of dimensions compared to \ourhash{} and SimHash, this happens for both cpu and gpu executions. So even though MinHash uses less dimensions to estimate the Jaccard it requires more time to estimate the Jaccard index.

